Notes on Local Grand Unification

Grand unified models in four dimensions typically suffer from the doublet-triplet splitting problem. This obstacle can be overcome in higher-dimensional settings, where a non-trivial gauge group topography can explain the simultaneous appearance of complete standard model generations in the form of 16-plets of SO(10) and the Higgs fields as split multiplets. In these notes, the emerging scheme of `local grand unification' and its realization in the context of orbifold compactifications of the heterotic string are reviewed.

==> pst-blur.tex <==
%%
%% This is file `pst-blur.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-blur.dtx  (with options: `texfile')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-blur.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-blur.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% $Id: pst-blur.dtx,v 2.0 2005/09/08 09:48:33 giese Exp $
%%
%% Copyright 1998-2007 Martin Giese, mgiese@risc.uni-linz.ac.at
%%                     Herbert Voss, voss@pstricks.de
%%
%% This file is under the LaTeX Project Public License
%% See CTAN archives in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-blur' is a PSTricks package for blurred shadows
%%
\csname PstBlurLoaded\endcsname
\let\PstBlurLoaded\endinput
\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }\expandafter\next
\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey \fi
%%
\def\fileversion{2.0}
\def\filedate{2005/09/08}
\message{ v\fileversion, \filedate}
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
\pst@addfams{pst-blur}
\pstheader{pst-blur.pro}
\newif\ifpsblur
\define@key[psset]{pst-blur}{blur}[true]{\@nameuse{psblur#1}\pst@setrepeatarrowsflag}
\psset{blur=false}
%%
\define@key[psset]{pst-blur}{blurradius}{\pst@getlength{#1}\psx@blurradius}
\psset{blurradius=1.5pt}
%%
\define@key[psset]{pst-blur}{blursteps}{\pst@getint{#1}\psx@blursteps}
\psset{blursteps=20}
%%
\define@key[psset]{pst-blur}{blurbg}{\pst@getcolor{#1}\psx@blurbg}
\psset{blurbg=white}
\def\pst@closedshadow{%
\ifpsblur\pst@blurclosedshadow\else\pst@sharpclosedshadow\fi
}
\def\pst@sharpclosedshadow{%
  \addto@pscode{%
    gsave
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    \tx@Shadow
    \pst@usecolor\psshadowcolor
    gsave fill grestore
    stroke
    grestore
    gsave
    \pst@usecolor\psfillcolor
    gsave fill grestore
    stroke
    grestore}}
\def\pst@blurclosedshadow{%
  \addto@pscode{%
    gsave
    gsave \pst@usecolor\psshadowcolor currentrgbcolor grestore
    gsave \pst@usecolor\psx@blurbg currentrgbcolor grestore
    \psx@blurradius\space
    \psx@blursteps\space
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    tx@PstBlurDict begin BlurShadow end
    grestore
    gsave
    \pst@usecolor\psfillcolor
    gsave fill grestore
    stroke
    grestore}}
\def\psblurbox{%
\def\pst@par{}\pst@object{psblurbox}}
\def\psblurbox@i{\pst@makebox\psblurbox@ii}
\def\psblurbox@ii{%
  \begingroup
  \pst@useboxpar
  \psblurtrue
  \psshadowtrue
  \psboxseptrue
  \setbox\pst@hbox=\hbox{\psframebox@ii}%
  \pst@dimh=\psk@shadowsize\p@
  \pst@dimh=.7071\pst@dimh
  \advance\pst@dimh\psx@blurradius\p@
  \pst@dimg=\dp\pst@hbox
  \advance\pst@dimg\pst@dimh
  \dp\pst@hbox=\pst@dimg
  \pst@dimg=\wd\pst@hbox
  \advance\pst@dimg\pst@dimh
  \wd\pst@hbox=\pst@dimg
  \leavevmode
  \box\pst@hbox
\endgroup}
%%
\catcode`\@=\TheAtCode\relax
\endinput
%%
%% End of file `pst-blur.tex'.


==> pst-slpe.tex <==
%%
%% This is file `pst-slpe.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-slpe.dtx  (with options: `texfile')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-slpe.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-slpe.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\def\pstslpefileversion{1.1}
\def\pstslpefiledate{2005/10/05}
\message{ v\pstslpefileversion, \pstslpefiledate}
\csname PstSlopeLoaded\endcsname
\let\PstSlopeLoaded\endinput
\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }\expandafter\next
\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey \fi % --> hv
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
\pst@addfams{pst-slpe}                              % --> hv
\pstheader{pst-slpe.pro}
\newrgbcolor{slopebegin}{0.9 1 0}
\define@key[psset]{pst-slpe}{slopebegin}{\pst@getcolor{#1}\psslopebegin}% --> hv
\psset[pst-slpe]{slopebegin=slopebegin}                                 % --> hv

\newrgbcolor{slopeend}{0 0 1}
\define@key[psset]{pst-slpe}{slopeend}{\pst@getcolor{#1}\psslopeend}% --> hv
\psset[pst-slpe]{slopeend=slopeend}% --> hv

\define@key[psset]{pst-slpe}{slopesteps}{\pst@getint{#1}\psslopesteps}% --> hv
\psset[pst-slpe]{slopesteps=100}% --> hv

\define@key[psset]{pst-slpe}{slopeangle}{\pst@getangle{#1}\psx@slopeangle}% --> hv
\psset[pst-slpe]{slopeangle=0}% --> hv
\define@key[psset]{pst-slpe}{slopecolors}{\def\psx@slopecolors{#1}}% --> hv
\psset[pst-slpe]{slopecolors={% --> hv
0.0 1 0 0
0.4 0 1 0
0.8 0 0 1
1.0 1 0 1
4}}
\define@key[psset]{pst-slpe}{slopecenter}{\def\psx@slopecenter{#1}}% --> hv
\psset[pst-slpe]{slopecenter={0.5 0.5}}% --> hv
\define@key[psset]{pst-slpe}{sloperadius}{\pst@getlength{#1}\psx@sloperadius}% --> hv
\psset[pst-slpe]{sloperadius=0}% --> hv
\def\psfs@slopes{%
 \addto@pscode{
  \psx@slopecolors\space
  \psslopesteps
  \psx@slopeangle
  tx@PstSlopeDict begin SlopesFill end}}
\def\psfs@slope{%
 \addto@pscode{%
  gsave
    0 \pst@usecolor\psslopebegin currentrgbcolor
    1 \pst@usecolor\psslopeend currentrgbcolor
    2
  grestore
  \psslopesteps \psx@slopeangle tx@PstSlopeDict begin SlopesFill end}}
\def\psfs@ccslopes{%
 \addto@pscode{%
  \psx@slopecolors\space
  \psslopesteps \psx@slopecenter\space \psx@sloperadius\space
  tx@PstSlopeDict begin CcSlopesFill end}}
\def\psfs@ccslope{%
 \addto@pscode{%
  gsave 0 \pst@usecolor\psslopebegin currentrgbcolor
    1 \pst@usecolor\psslopeend currentrgbcolor
    2 grestore
  \psslopesteps \psx@slopecenter\space \psx@sloperadius\space
  tx@PstSlopeDict begin CcSlopesFill end}}
\def\psfs@radslopes{%
 \addto@pscode{%
  \psx@slopecolors\space
  \psslopesteps\psx@slopecenter\space\psx@sloperadius\space\psx@slopeangle
  tx@PstSlopeDict begin RadSlopesFill end}}
\def\psfs@radslope{%
 \addto@pscode{%
  gsave 0 \pst@usecolor\psslopebegin currentrgbcolor
    1 \pst@usecolor\psslopeend currentrgbcolor
    2 \pst@usecolor\psslopebegin currentrgbcolor
    3 \pst@usecolor\psslopeend currentrgbcolor
    4 \pst@usecolor\psslopebegin currentrgbcolor
    5 grestore
  \psslopesteps\psx@slopecenter\space\psx@sloperadius\space\psx@slopeangle
  tx@PstSlopeDict begin RadSlopesFill end}}

\catcode`\@=\TheAtCode\relax
\endinput
%%
%% End of file `pst-slpe.tex'.

